In-Depth Exploration of Single-Snapshot Lossy Compression Techniques for N-Body Simulations

In situ lossy compression allowing user-controlled data loss can significantly reduce the I/O burden. For large-scale N-body simulations where only one snapshot can be compressed at a time, the lossy compression ratio is very limited because of the fairly low spatial coherence of the particle data. In this work, we assess the state-of-the-art single-snapshot lossy compression techniques of two common N-body simulation models: cosmology and molecular dynamics. We design a series of novel optimization techniques based on the two representative real-world N-body simulation codes. For molecular dynamics simulation, we propose three compression modes (i.e., best speed, best tradeoff, best compression mode) that can refine the tradeoff between the compression rate (a.k.a., speed/throughput) and ratio. For cosmology simulation, we identify that our improved SZ is the best lossy compressor with respect to both compression ratio and rate. Its compression ratio is higher than the second-best compressor by 11% with comparable compression rate. Experiments with up to 1024 cores on the Blues supercomputer at Argonne show that our proposed lossy compression method can reduce I/O time by 80% compared with writing data directly to a parallel file system and outperforms the second-best solution by 60%. Moreover, our proposed lossy compression methods have the best rate-distortion with reasonable compression errors on the tested N-body simulation data compared with state-of-the-art compressors.

==> tex/character.tex <==
\section{In-depth Understanding of N-body simulation Data Sets}
\label{sec: character}

%To better understand why a certain lossy compressor can achieve better compression quality than the others can, one must understand the characteristics of the data.  
In this section, we use the HACC and AMDF data sets as examples to understand the data characteristics of N-body simulations and explore the reason why a certain lossy compressor can achieve better compression quality than the others can. 
We first provide a visualization of each field/variable in the HACC and AMDF data sets.
We then further analyze their potential statistical features.

\subsection{Visual Analysis of N-body Simulation Data Sets}
\label{subsec: vis-analysis}

\begin{figure}[t]
\centering
\includegraphics[scale=0.46]{fig/Fig11.pdf}
\caption{Partial visualization of coordinate variables and velocity variables in HACC and AMDF data sets.}
\label{fig:fig11}
\vspace{-2mm}
\end{figure}

%\begin{figure*}
%\centering
%   \begin{subfigure}[b]{0.4\textwidth}
%        \centering
%   \includegraphics[width=0.4\textwidth]{fig/Fig1a.pdf}
%   \caption{Coordinate variables}
%   \label{fig:fig1a} 
%\end{subfigure}
%
%\begin{subfigure}[b]%{0.4\textwidth}
%     \centering
%   \includegraphics[width=0.4\textwidth]{fig/Fig1b.pdf}
%   \caption{Velocity variables}
%   \label{fig:fig1b}
%\end{subfigure}


%\begin{subfigure}[b]{0.4\textwidth}
%     \centering
%   \includegraphics[width=\textwidth]{fig/Fig6a.pdf}
%   \caption{Coordinate variables}
%   \label{fig:fig6a} 
%\end{subfigure}
%
%\begin{subfigure}[b]{0.4\textwidth}
%     \centering
%   \includegraphics[width=\textwidth]{fig/Fig6b.pdf}
%   \caption{Velocity variables}
%   \label{fig:fig6b}
%\end{subfigure}

%\caption{Partial visualization of (a) coordinate variables and (b) velocity variables in HACC data sets.}
%\label{fig:fig1}
%\vspace{-4mm}
%\end{figure*}

%\begin{figure}
%\centering
%   \begin{subfigure}[b]{0.4\textwidth}
%   \includegraphics[width=\textwidth]{fig/Fig6a.pdf}
%   \caption{Coordinate variables}
%   \label{fig:fig6a} 
%\end{subfigure}
%
%\begin{subfigure}[b]{0.4\textwidth}
%   \includegraphics[width=\textwidth]{fig/Fig6b.pdf}
%   \caption{Velocity variables}
%   \label{fig:fig6b}
%\end{subfigure}
%
%\caption{Partial visualization of (a) coordinate variables and (b) velocity variables in AMDF data sets.}
%\label{fig:fig6}
%\vspace{-2mm}
%\end{figure}

Figure \ref{fig:fig11} (a) and (b) shows what the six 1D variables $xx$, $yy$, $zz$, $vx$, $vy$, $vz$ in the HACC data sets, including the partial visualization of coordinate variables and velocity variables separately. For coordinate variables of the HACC data sets, Figure \ref{fig:fig11} (a) indicates that the values of $xx$ and $yy$ exhibit an increasing trend over a wide index range, for example, $[1 \cdot 10^6, 2 \cdot 10^6]$. Unlike $xx$ and $yy$, the $zz$ values increase periodically in a very short index range such as $[1.0002 \cdot 10^6, 1.0008 \cdot 10^6]$, as shown in Figure \ref{fig:fig11} (b). We also note that $xx$ has a smaller variance than $yy$ has. Although $zz$ exhibits a strong periodical change, it has a diverse changing cycle (in the range of [500,1000+]) that cannot be predicted accurately. Unlike the coordinate variables in the AMDF data sets, its velocity data look  irregular and random without such visible patterns.

We present the data of the AMDF simulation in Figure \ref{fig:fig11} (c) and (d). Unlike HACC data, both the coordinate and velocity variables in AMDF look irregular and random, and the velocity data span a large value range. 

Based on this visual analysis, we can organize the data variables in the order of decreasing regularity as follows: $coord_{hacc}$, $vel_{hacc}$, $coord_{amdf}$, $vel_{amdf}$. Here $coord_{hacc}$, $vel_{hacc}$, $coord_{amdf}$, $vel_{amdf}$ represent the coordinates in the HACC data sets, velocities in the HACC data sets, coordinates in the AMDF data sets, and velocities in the AMDF data sets, respectively.

\subsection{In-Depth Statistical Analysis of N-Body Simulation Data}
\label{subsec: stat-analysis}
We next analyze the data sets statistically and explore the relation between compression ratios of different compression methods and data characteristics.

\begin{table}[]
\centering
\caption{Autocorrelation analysis of different variables in HACC and AMDF data sets}
\label{tab: autocorr}
\begin{adjustbox}{width=\columnwidth}
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
              & \textbf{xx} & \textbf{yy} & \textbf{zz} & \textbf{vx} & \textbf{vy} & \textbf{vz} \\ \hline
\textbf{HACC} & 0.9999972   & 0.99998     & 0.98        & 0.92        & 0.92        & 0.92        \\ \hline
\textbf{AMDF} & 0.76        & 0.75        & 0.64        & -0.0002     & -0.0003     & 0.0002      \\ \hline
\end{tabular}
\end{adjustbox}
\vspace{-2mm}
\end{table}


%\begin{table}[]
%\centering
%\caption{Autocorrelation analysis of different variables in HACC data sets}
%\label{tab: autocorr-hacc}
%\begin{adjustbox}{width=0.75\columnwidth}
%\begin{tabular}{|l|c|c|c|c|c|c|}
%\hline
%\textbf{Delay} & \textbf{xx} & \textbf{yy} & \textbf{zz} & \textbf{vx} & \textbf{vy} & \textbf{vz} \\ \hline
%1              & 0.9999972   & 0.99998     & 0.98        & 0.92    & 0.92 & 0.92    \\ \hline
%2              & 0.9999968   & 0.99995     & 0.97        & 0.89    & 0.89 & 0.88    \\ \hline
%4              & 0.9999966   & 0.99991     & 0.95        & 0.85    & 0.86 & 0.83    \\ \hline
%8              & 0.9999963   & 0.99982     & 0.91        & 0.79    & 0.80 & 0.75    \\ \hline
%16             & 0.9999960   & 0.99965     & 0.82        & 0.68    & 0.71 & 0.62    \\ \hline
%32             & 0.9999955   & 0.99931     & 0.66        & 0.53    & 0.57 & 0.44    \\ \hline
%64             & 0.9999947   & 0.99864     & 0.39        & 0.33    & 0.39 & 0.23    \\ \hline
%\end{tabular}
%\end{adjustbox}
%\vspace{-2mm}
%\end{table}

%\begin{table}[]
%\centering
%\caption{Autocorrelation analysis of different variables in AMDF data sets}
%\label{tab: autocorr-amdf}
%\begin{adjustbox}{width=0.75\columnwidth}
%\begin{tabular}{|l|c|c|c|c|c|c|}
%\hline
%\textbf{Delay} & \textbf{xx} & \textbf{yy} & \textbf{zz} & \textbf{vx} & \textbf{vy} & \textbf{vz} \\ \hline
%1              & 0.76   & 0.75     & 0.64        & -0.0002    & -0.0003 & 0.0002    \\ \hline
%2              & 0.64   & 0.66     & 0.49        & 0.0007    & -0.0003 & -0.0004    \\ \hline
%4              & 0.69   & 0.70     & 0.57        & 0.0005    & 0.0006 & 0.0006    \\ \hline
%8              & 0.67   & 0.67    & 0.54           & -0.0006 & 0.0007 & 0.0007    \\ \hline
%16             & 0.64   & 0.64     & 0.53       & -0.0005    & -0.0009 & 6.3E-06    \\ \hline
%32             & 0.56   & 0.56     & 0.46        & 0.0007    & 0.0009 & 0.0002    \\ \hline
%64             & 0.40   & 0.40     & 0.31        & 0.0005    & 0.0010 & -0.0007    \\ \hline
%\end{tabular}
%\end{adjustbox}
%\vspace{-2mm}
%\end{table}


% \begin{table}[]
% \centering
% \caption{Autocorrelation analysis of different variables in HACC data sets}
% \label{tab: autocorr-exaalt}
% \begin{tabular}{|l|c|c|c|c|}
% \hline
% \textbf{Delay} & \textbf{xx} & \textbf{yy} & \textbf{zz} & \textbf{vx} \\ \hline
% 1              & 0.9999972   & 0.99997     & 0.98        & 0.92        \\ \hline
% 2              & 0.9999968   & 0.99995     & 0.97        & 0.89        \\ \hline
% 4              & 0.9999966   & 0.99991     & 0.95        & 0.85        \\ \hline
% 8              & 0.9999963   & 0.99982     & 0.91        & 0.79        \\ \hline
% 16             & 0.9999960   & 0.99965     & 0.82        & 0.68        \\ \hline
% 32             & 0.9999955   & 0.99931     & 0.66        & 0.53        \\ \hline
% 64             & 0.9999947   & 0.99864     & 0.39        & 0.33        \\ \hline
% \end{tabular}
% \end{table}

\begin{table}[]
\centering
\vspace{-1mm}
\caption{Compression ratios of different variables with different compressors on HACC data sets under $eb_{rel} = 10^{-4}$}
\label{tab: varcr-hacc}
\begin{adjustbox}{width=0.7\columnwidth}
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
\textbf{Compressor} & \textbf{xx} & \textbf{yy} & \textbf{zz} & \textbf{vx} & \textbf{vy} & \textbf{vz} \\ \hline
CPC2000             & 7.1         & 7.1         & 7.1         & 2.3    &   2.3  & 2.3 \\ \hline
FPZIP               & 5.8         & 5.7         & 4.4         & 2.2    &   2.2  & 2.2 \\ \hline
ZFP                 & 2.3         & 2.3         & 2.2         & 2.3   &  2.3    & 2.3 \\ \hline
SZ                  & 6.9         & 6.8         & 5.3         & 3.7   &  3.6    & 3.6 \\ \hline
\end{tabular}
\end{adjustbox}
%\vspace{-4mm}
\end{table}


\begin{table}[]
\centering
\vspace{-2mm}
\caption{Compression ratios of different variables with different compressors on AMDF data sets under $eb_{rel} = 10^{-4}$}
\label{tab: varcr-amdf}
\begin{adjustbox}{width=0.7\columnwidth}
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
\textbf{Compressor} & \textbf{xx} & \textbf{yy} & \textbf{zz} & \textbf{vx} & \textbf{vy} & \textbf{vz} \\ \hline
CPC2000             & 5.5         & 5.5         & 5.5         & 2.3    &   2.3  & 2.3 \\ \hline
FPZIP               & 1.9         & 2.3         & 2.0         & 1.7    &   1.7  & 1.7 \\ \hline
ZFP                 & 2.0         & 1.9         & 1.9         & 1.9   &  1.9    & 1.9 \\ \hline
SZ                  & 2.8         & 2.8         & 2.7         & 2.5   &  2.5    & 2.5 \\ \hline
\end{tabular}
\end{adjustbox}
\vspace{-6mm}
\end{table}

We analyze the autocorrelation of each variable in the HACC and AMDF data sets. Table \ref{tab: autocorr} shows the autocorrelation coefficients of each variable in the HACC and AMDF data sets. The table illustrates that the $coord_{hacc}$ has the strongest autocorrelation and the $vel_{amdf}$ has the weakest autocorrelation, which is consistent with our visual analysis. We also present the breakdown of compression ratios of the coordinate and velocity variables using different compressors on the HACC and AMDF data sets under the value-range-based relative error bound $10^{-4}$ in Tables \ref{tab: varcr-hacc} and \ref{tab: varcr-amdf}. Based on Tables \ref{tab: varcr-hacc} and \ref{tab: varcr-amdf}, we make several observations as follows.

\begin{enumerate}[noitemsep,topsep=0pt]
%\item For FPZIP and SZ, the stronger the autocorrelation that the variable has, the higher the compression ratio that they can achieve on the variable.
\item For CPC2000,  much higher compression ratios can be achieved on the coordinate variables than on the velocity variables.
\item For the HACC data sets, SZ's compression ratios are close to those of CPC2000's on the coordinate variables but are about 60\% higher than CPC2000's on the velocity variables.
\item For the AMDF data sets, SZ's compression ratios are close to those of CPC2000 on the velocity variables, but are about 50\% lower than CPC2000's on the coordinate variables.
\end{enumerate}

%For observation (1), SZ lossy compressor adopts multilayer prediction model \cite{sz17} and FPZIP adopts Lerenzo predictor \cite{fpzip}. Both  prediction models will gracefully degrade to linear-curve fitting or last-value fitting when the dimensional size is set to 1. The autocorrelation can reflect the degree of linear correlation between adjacent data points, which can well explain that FPZIP and SZ can achieve higher prediction accuracy and compression ratio on the data sets with higher autocorrelations.

For observation (1), CPC2000 performs a sorting, based on the spatial locality information, namely, R-index-based sorting \cite{cpc2000}. We will discuss the details of R-index-based sorting in Section \ref{sec: optimization}. After R-index-based sorting, the data with closer locality in space will be processed/compressed more concentratedly. Hence, it  can achieve better compression ratios on the spatial relevant data (i.e., coordinate variables) in particular. 

For observation (2), on the HACC data sets, SZ has  compression ratios similar to those of CPC2000 on the coordinate variables because of $xx, yy, zz$'s extremely high autocorrelation (i.e., more than 0.98). Also, SZ has higher compression ratios than CPC2000 has on the velocity variables because $vx, vy, vz$ in the HACC data sets have high autocorrelation (i.e., 0.92). After R-index-based sorting, however, the velocity variables lose their initial good correlation. We will show the details in Section 5.3. Therefore, the overall compression ratio of CPC2000 (i.e., 3.5) is 24\% lower than that of SZ (i.e, 4.6).

For observation (3), on the AMDF data sets, because of the extremely low autocorrelation, the values of the velocity variables can be seen as fairly random; hence, the R-index-based sorting will not affect the velocity variables much. Consequently, R-index can improve the compression ratios on the coordinate variables without reducing the ratios on the velocity variables, and hence, CPC2000 can outperform the best-solution SZ by about 22\%.

Note that the above observations and analysis are also applicable to the other cosmology and molecular dynamics simulations due to the representativeness of the HACC and AMDF data sets, as confirmed by HACC and AMDF team. Therefore, in the following section, we will propose a series of novel optimization techniques based on these observations and analysis to improve the lossy compression on N-body simulation data sets.
